The Websky Extragalactic CMB Simulations

We present a new pipeline for the efficient generation of synthetic observations of the extragalactic microwave sky, tailored to large ground-based CMB experiments such as the Simons Observatory, Advanced ACTPol, SPT-3G, and CMB-S4. Such simulated observations are a key technical challenge in cosmology because of the dynamic range and accuracy required. The first part of the pipeline generates a random cosmological realization in the form of a dark matter halo catalog and matter displacement field, as seen from a given position. The halo catalog and displacement field are modeled with ellipsoidal collapse dynamics and Lagrangian perturbation theory, respectively. In the second part, the cosmological realization is converted into a set of intensity maps over the range 10 - 10^3 GHz using models based on existing observations and hydrodynamical simulations. These maps include infrared emission from dusty star forming galaxies (CIB), Comptonization of CMB photons by hot gas in groups and clusters through the thermal Sunyaev-Zel'dovich effect (tSZ), Doppler boosting by Thomson scattering of the CMB by bulk flows through the kinetic Sunyaev-Zel'dovich effect (kSZ), and weak gravitational lensing of primary CMB anisotropies by the large-scale distribution of matter in the universe. After describing the pipeline and its implementation, we present the Websky maps, created from a realization of the cosmic web on our past light cone in the redshift interval 0<z<4.6 over the full-sky and a volume of ~(600 Gpc/h)^3 resolved with ~10^12 resolution elements. The Websky maps and halo catalog are publicly available at mocks.cita.utoronto.ca/websky.

==> extra_text.tex <==
OLD
The Planck collaboration presented the cross-correlation of Compton-y maps reconstructed from their SZ-detected sample, PSZ2 \cite{2016A&A...594A..27P}, with their temperature maps at different frequencies, $C_\ell^{y_cT_\nu}$, where $y_c$ is the $y$--parameter obtained by assuming each cluster follows the analytical Planck universal pressure profile corresponding to its measured SZ parameters. These measurements are shown as points with error bars in Figure \ref{fig:cib-tsz}. The units used for intensity are "Compton $y$-units" \cite{2014A&A...571A..29P}, defined for each bandpass $i$ such that 
\beq
y_i = I_{\nu_i} / |d\Delta{I_\nu}/dy|_i,
\eeq
with conversion factors taken from Table 6 of \cite{2014A&A...571A..29P}. See \cite{2016A&A...594A..23P} for more details on how the cross-correlation was calculated. 

We have followed a similar procedure with our simulated tSZ and CIB maps, in order to test consistency of our CIB maps. We first determined an approximate selection function using a hard minimum mass boundary as a function of redshift, including only halos in our lightcone satisfying $M_{500}>M_{\rm psz2}(z)$, where we have fit to the 50\% completeness curve from the left panel in Figure 26 of \cite{2016A&A...594A..23P} with $M_{\rm psz2}(z)=6.8(z^3 - 2.7z^2 + 2.5z + 0.1) 10^{14}M_\odot$.

%27., 39., 93., 100., 143., 145., 217., 225., 280., 353., 545., 857.

% 45.49453276,  22.253273  ,   4.68307475,   4.18768454, 2.63201885,   2.59470195,   2.06761653,   2.07161949, 2.33024461,   3.37095843,  17.50814263, 696.53489997

% -5.34870711e+06, -5.23843653e+06, -4.28400198e+06, -4.11032686e+06, -2.83550980e+06, -2.76848729e+06, -2.11880760e+04,  3.15165361e+05, 2.73143205e+06,  6.10714949e+06,  1.52574383e+07,  3.02275497e+07

% %BEGIN FIGURE -------------
% \begin{figure*}
% \vspace{0.3cm}
% \begin{center}
% \includegraphics[width=0.5\textwidth,trim={700 0 0 0},clip]{Figures/Algorithm/algorithm.pdf}
% \includegraphics[width=0.43\textwidth,trim={0 0 750 0},clip]{Figures/Algorithm/algorithm.pdf}
% \end{center}
% \vspace{-0.3cm}
% \mycap{Schematic representation of the simulation pipeline.}
% \label{fig:algorithm}
% \end{figure*}
% %END FIGURE ----------------





%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%BEGIN FIGURE -------------
% \begin{figure}
% \begin{center}
% \includegraphics[width=0.34\textwidth, trim = 0 0 0 0, clip = True]{Figures/HaloStatistics/hmf.pdf}
% %\hfill
% \includegraphics[width=0.65\textwidth, trim = 10 0 0 0, clip = True]{Figures/HaloStatistics/top.pdf}
% \end{center}
% \vspace{-0.8cm}
% \caption{{\em Left}: Halo abundance in redshift intervals on the light cone. Mean values are shown as thick lines, with intervals as labelled, and a sample of 40 individual realizations shown as thin lines. {\em Center}: The cumulative distribution of redshift of the most massive halo in each realization, along with the median and $\pm$1$\sigma$ values in the distribution as solid and dotted black vertical lines, respectively. {\em Right}: Same as center, but for halo mass. In each of the right two panels, median and $\pm$1$\sigma$ values reported by \cite{2012ApJ...755L..36H} are shown in red, and are in good agreement with our results.}
% \label{fig:hmf}
% \end{figure}
%END FIGURE ----------------

%BEGIN FIGURE -------------
% \begin{figure}[t]
% \begin{center}
% \includegraphics[width=0.48\textwidth, trim = 0 0 0 -10, clip = True]{Figures/PowerSpectra/ComptonBBPS.pdf}
% \hfill
% \includegraphics[width=0.48\textwidth, trim = 0 0 0 0, clip = True]{Figures/tsz_auto_planck.pdf}
% \vspace{-0.5cm}
% \end{center}
% \caption{Left: Comparison of Peak Patch and BBPS power spectra. Light curves show the power spectra from all fully sky realizations, while the thick solid lines indicate the mean. Dotted are the 'profile paste' power spectra from BBPS (see \cite{2012ApJ...758...75B} for more details of how those power spectra were computed). Right: Angular power spectrum of the Compton--$y$ parameter for maps obtained from a random selection of 50 light cone simulations (grey) as well as median (solid), 1--$\sigma$ (dotted), and 2--$\sigma$ (dashed) contours for all 320 simulations. The points from the power spectrum of the Planck $y$--map have been shifted downward by a factor of $(0.25/0.3)^3$ to approximately compensate for the low value of $\Omega_m=0.25$ we used in our simulations relative to the best fit Planck cosmology.}
% \label{fig:tsz-lowz}
% \end{figure}
%END FIGURE ----------------

%BEGIN FIGURE -------------
% \begin{figure}[t]
% \begin{center}
% \includegraphics[width=0.48\textwidth, trim = 0 0 0 -10, clip = True]{Figures/PowerSpectra/ComptonBBPS.pdf}
% \hfill
% \includegraphics[width=0.48\textwidth, trim = 0 0 0 0, clip = True]{Figures/tsz_auto_planck.pdf}
% \vspace{-0.5cm}
% \end{center}
% \caption{Left: Comparison of Peak Patch and BBPS power spectra. Light curves show the power spectra from all fully sky realizations, while the thick solid lines indicate the mean. Dotted are the 'profile paste' power spectra from BBPS (see \cite{2012ApJ...758...75B} for more details of how those power spectra were computed). Right: Angular power spectrum of the Compton--$y$ parameter for maps obtained from a random selection of 50 light cone simulations (grey) as well as median (solid), 1--$\sigma$ (dotted), and 2--$\sigma$ (dashed) contours for all 320 simulations. The points from the power spectrum of the Planck $y$--map have been shifted downward by a factor of $(0.25/0.3)^3$ to approximately compensate for the low value of $\Omega_m=0.25$ we used in our simulations relative to the best fit Planck cosmology.}
% \label{fig:tsz-lowz}
% \end{figure}
%END FIGURE ----------------

%BEGIN FIGURE -------------
% \begin{figure}[t]
% \begin{center}
%\includegraphics[width=0.3\textwidth, trim = 150 0 0 0, clip = True]{Figures/Analytics/dlnInudlnMdz.pdf}

% \includegraphics[width=0.98\textwidth, trim = 5 0 0 0, clip = True]{Figures/PowerSpectra/cib_x_tsz/CIB_x_tSZ_w_planck.pdf}
% \end{center}
% \vspace{-0.5cm}
% \caption{
% %{\bf{Left}}:Contribution to mean intensity to CIB of dusty star forming galaxies as a function of redshift and halo mass. {\bf{Right}} 
% The cross-correlation of a Compton-$y$ map containing only the most massive clusters in one of our light cones, meant to follow the PSZ2 cluster mass and redshift selection function, with the total intensity as modeled from the total CIB and tSZ signals from the same simulation, at different frequencies. The blue curve is tSZ auto for the full sky map, green is tSZ auto for the PSZ2 cut, and red is for the full CIB x PSZ2 cut. Compton-$y$ units are used throughout (see text).}
% \label{fig:cib-tsz}
% \end{figure}
%END FIGURE ---------------

%BEGIN FIGURE -------------
%\begin{figure}[t]
%\begin{center}
%\includegraphics[width=0.3\textwidth, trim = 150 0 0 0, clip = True]{Figures/Analytics/dlnInudlnMdz.pdf}
%\includegraphics[width=0.98\textwidth, trim = 5 0 0 0, clip = True]{Figures/PowerSpectra/cib_x_tsz/CIB_x_tSZ_w_planck.pdf}
%\end{center}
%\vspace{-0.5cm}
%\caption{
%{\bf{Left}}:Contribution to mean intensity to CIB of dusty star forming galaxies as a function of redshift and halo mass. {\bf{Right}} 
%\label{fig:cib-tsz}
%\end{figure}
%END FIGURE ---------------



%BEGIN FIGURE -------------
% \begin{figure}[t]
% \begin{center}
% \includegraphics[width=0.29\textwidth, trim = 0 -20 0 0, clip = True]{Figures/PowerSpectra/cmb_lensing/clkappa_new.pdf}
% \includegraphics[width=0.65\textwidth, trim = 0 0 0 0, clip = True]{Figures/PowerSpectra/cmb_lensing/cmb_cl_lensed_unlensed_difference_ell4000.pdf}
% \vspace{-0.5cm}
% \end{center}
% \caption{Left: CMB Lensing convergence power spectrum. The solid blue is of the map containing halos only, the solid red is the map containing the field, while the black is of the total. The dotted curves show the Limber approximation applied to the linear matter power spectrum (red), the nonlinear one from Halo Fit (black), and the difference between the two -- i.e. the nonlinear correction (blue). Middle: The TT (blue), EE (red) and BB (blue) power spectra, before (thin) and after (thick) lensing by the CMB $\kappa$ map. Right: Relative differences between lensed and unlensed power spectra for TT (top) and EE (bottom), using the theoretical calculation in CAMB (solid) and the power spectra from the simulated maps (dashed).}
% \label{fig:lensing-validation}
% \end{figure}
%END FIGURE ----------------

% \section{Appendix A: Halo/Field Decomposition}
% \label{sec:halofieldappendix}

% %BEGIN FIGURE -------------
% \begin{figure}[t]
% \begin{center}
% \includegraphics[width=1.0\textwidth, trim = -70 0 0 0, clip = True]{Figures/HaloField/halofield_imshow.pdf}
% \includegraphics[width=0.45\textwidth, trim = 0 0 0 0, clip = True]{Figures/HaloField/pk_halofield_k.pdf}}
% \includegraphics[width=0.45\textwidth, trim = 0 0 0 0, clip = True]{Figures/HaloField/pk_halofield_ell.pdf}}
% \vspace{-0.7cm}
% \end{center}
% \caption{Halo Field}
% \label{fig:halofield}
% \end{figure}
% %END FIGURE ----------------

